On lattice-free boosted MMI training of HMM and CTC-based full-context ASR models

Hybrid automatic speech recognition (ASR) models are typically sequentially trained with CTC or LF-MMI criteria. However, they have vastly different legacies and are usually implemented in different frameworks. In this paper, by decoupling the concepts of modeling units and label topologies and building proper numerator/denominator graphs accordingly, we establish a generalized framework for hybrid acoustic modeling (AM). In this framework, we show that LF-MMI is a powerful training criterion applicable to both limited-context and full-context models, for wordpiece/mono-char/bi-char/chenone units, with both HMM/CTC topologies. From this framework, we propose three novel training schemes: chenone(ch)/wordpiece(wp)-CTC-bMMI, and wordpiece(wp)-HMM-bMMI with different advantages in training performance, decoding efficiency and decoding time-stamp accuracy. The advantages of different training schemes are evaluated comprehensively on Librispeech, and wp-CTC-bMMI and ch-CTC-bMMI are evaluated on two real world ASR tasks to show their effectiveness. Besides, we also show bi-char(bc) HMM-MMI models can serve as better alignment models than traditional non-neural GMM-HMMs.

==> 1_state_topo.tex <==
\setlength{\mynodehorsep}{0.2\columnwidth}
\setlength{\mynodeversep}{0.1\columnwidth}
\centering
\tikzset{every state/.style={minimum size=0pt}}

\begin{tikzpicture}  [auto,
    initial/.style={line width=.1pt},
    accepting by double/.append style={},
    semithick,
    node distance = \mynodehorsep,
    label/.style={above, sloped, midway},
    loopslant/.style={out = 105, in = 75, looseness = 8, min distance = 0.1in}
  ]
  \node[state,initial, minimum size=0, inner sep=0] (qs) at (-1, 0) {};
  \node[state] (q0) at (0,0) {0};
  \node[state] (q1) at (1,0) {1};
\node[state] (q2) at (2,0) {2};
\node[state] (q3) at (3,0) {3};
\node[state] (q4) at (4,0) {4};
\node[state, accepting] (q5) at (5,0) {5};
\draw[-angle 60] (qs) edge node[auto, swap] {} (q0);
\draw[-angle 60] (q0) edge node[auto, swap] {I:I} (q1);
\draw[-angle 60] (q1) edge node[auto, swap] {sil:sil} (q2);
\draw[-angle 60] (q2) edge node[auto, swap] {$_a:_a$} (q3);
\draw[-angle 60] (q3) edge node[auto, swap] {$m:m$} (q4);
\draw[-angle 60] (q4) edge node[auto, swap] {$sil:sil$} (q5);
\end{tikzpicture}

==> rebuttal.tex <==
**0CA0**
Importance/Relevance	Of sufficient interest
Justification of Importance/Relevance Score
[None Provided by Reviewer]
Novelty/Originality/Contribution	Minor originality
Justification of Novelty/Originality/Contribution Score
While the authors provide a unified view for hybrid acoustic modeling, technical novelty is limited in combining existing algorithms.
The systematic experiments will be practically useful.
Technical Correctness	Probably correct
Justification of Technical Correctness Score
[None Provided by Reviewer]
Experimental Validation	Sufficient validation/theoretical paper
Justification of Experimental Validation Score
[None Provided by Reviewer]
Clarity of Presentation	Clear enough
Justification of Clarity of Presentation Score
* In Section 6.1.5, the meaning of the last sentence (This makes sense because...) is not clear to me.

* Why do you attach the period after "Table" (i.e., "Table. 1" should be "Table 1")?

* Section 5, 1st sentence: There is a typo at "model with a the degenerative version".

Reference to Prior Work	References adequate

**0D3E**

Importance/Relevance	Of limited interest
Justification of Importance/Relevance Score
Very specialized paper, of interest to hybrid model training practitioners.  
Novelty/Originality/Contribution	Minor originality
Justification of Novelty/Originality/Contribution Score
Mostly permutations of known approaches.
Technical Correctness	Probably correct
Justification of Technical Correctness Score
[None Provided by Reviewer]
Experimental Validation	Limited but convincing
Justification of Experimental Validation Score
[None Provided by Reviewer]
Clarity of Presentation	Difficult to read
Justification of Clarity of Presentation Score
Very dense. Hard to read for non-specialists in this subfield.  What's the take-home message?
Reference to Prior Work	References adequate
Justification of Reference to Prior Work
[None Provided by Reviewer]
Additional comments to author(s)
[None Provided by Reviewer]

**0F11**
Importance/Relevance	Of broad interest
Justification of Importance/Relevance Score
The paper gives significant insight into the effect of the label topologies on the performance of hybrid-asr systems. A lot of interesting conclusions can be drawn from the experiments found in this paper.
Novelty/Originality/Contribution	Moderately original
Justification of Novelty/Originality/Contribution Score
The novelty of this paper stems from the set of experiments done and the associated analysis. The different label topologies of hybrid asr systems have not been compared in this depth before.
Technical Correctness	Definitely correct
Justification of Technical Correctness Score
[None Provided by Reviewer]
Experimental Validation	Sufficient validation/theoretical paper
Justification of Experimental Validation Score
[None Provided by Reviewer]
Clarity of Presentation	Clear enough
Justification of Clarity of Presentation Score
[None Provided by Reviewer]
Reference to Prior Work	References adequate
Justification of Reference to Prior Work
[None Provided by Reviewer]
Additional comments to author(s)
Questions to the authors:
Sec 6.1: What is your definition of stride here? I guess you mean the ratio of input frames to output labels, but do you use all input frames or skip some? Also if you are already mentioning the stride you could also mention your frame-frequency (100Hz I guess).

Sec 6.1.4: When you measure the TSE, how is the time-stamp defined? An aligned word has a start and an end time, so how do you calculate the TSE exactly?

Sec 6.3: I think you should explain how to calculate the CE columns in Table 11 a little more. It's only one long sentence and that makes it a little difficult to read, especially given that this is not an established method.

Definite accept.


%-------------------------------------

Rebuttal

Thanks for the detailed reviews.

> Re comments on "Novelty/Originality/Contribution":

We want to politely point out that, rather than simply combining existing algorithms/know approaches, the experiments on the novel modeling approaches were enabled by building a framework by
1) Clearly decomposing the concepts of modeling units and label topologies, which establishes new understandings to the ASR community: Rather than being "CTC loss", "CTC" should more precisely refer to the label topology (comparable to HMM) of modeling units used in either ML or (LF-)MMI training. 
2) Proposing novel algorithms to build numerator/denominator FST for the CTC case, which are technically non-trivial, especially the chenone-CTC case. 

On one hand, this work enables, for the first time, a fair comparison of HMM and CTC topologies with exactly the same set of (wordpiece/chenone) modeling units, with both experiments designed and theories provided to explain their differences in WER/time-stamp accuracy performance, and interaction with SpecAugment. On the other hand, in practice, the framework gave birth to novel modeling approaches like wordpiece-CTC-MMI and chenone-CTC-MMI which show better WERs on real-world ASR tasks, and wordpiece-HMM-MMI which retains good time-stamp accuracy while allowing faster inference with larger stride. Besides, the bc-HMM-MMI as a novel approach for alignment model training, shown to work better than GMM, can be adopted to significantly simplify and improve reproducibility for any from-scratch ASR modeling pipeline.


> Re: "additional comments" from 0CA0:
1) Thanks for pointing out the confusion in Section 6.1.5. We'll rephrase the last sentence as:
We believe the reason behind the observation is that: The richer representation provided by chain topology, better modeling intra-class variations, contributes more to longer modeling units (wordpieces are longer than chenones).

2) Thanks for catching the period after Table. We will remove the period. We will also remove the extra article type in "model with a the degenerative version".

> Re: "additional comments" from OF11:
1)Stride is the ratio of input frame rate to output frame rate. Input frame rate is 100Hz i.e. frame shift of 10ms. The output rate is 25Hz for stride 4 models etc. We use all the input frames. For TDNN-BLSTM models, we subsample activations at intermediate TDNN layers (e.g. after 3 layers) by skipping some frames. For the transformer models, we stack 8 input feature frames and project it to 768 dim so the rest of network is at frame rate of 12.5Hz as mentioned in section 6.2.1.

2) We take the RMS of start and end time stamps. We will make this clearer in Section 6.1.4.

3) We will make this more clearer in that section. For training chenone hybrid models using CE, we need frame-level chenone labels for targets. In table 11, we compare obtaining these labels from two sources -- the HMM-GMM model (baseline approach), bc-HMM-MMI neural network model (proposed), and then evaluate the performance of the chenone hybrid model trained using those labels and report it in the column CE.
